Towards a Decomposition-Optimal Algorithm for Counting and Sampling Arbitrary Motifs in Sublinear Time

We consider the problem of sampling and approximately counting an arbitrary given motif $H$ in a graph $G$, where access to $G$ is given via queries: degree, neighbor, and pair, as well as uniform edge sample queries. Previous algorithms for these tasks were based on a decomposition of $H$ into a collection of odd cycles and stars, denoted $\mathcal{D}^*(H)=\{O_{k_1}, \ldots, O_{k_q}, S_{p_1}, \ldots, S_{p_\ell}\}$. These algorithms were shown to be optimal for the case where $H$ is a clique or an odd-length cycle, but no other lower bounds were known. We present a new algorithm for sampling and approximately counting arbitrary motifs which, up to $\textrm{poly}(\log n)$ factors, is always at least as good as previous results, and for most graphs $G$ is strictly better. The main ingredient leading to this improvement is an improved uniform algorithm for sampling stars, which might be of independent interest, as it allows to sample vertices according to the $p$-th moment of the degree distribution. Finally, we prove that this algorithm is \emph{decomposition-optimal} for decompositions that contain at least one odd cycle. These are the first lower bounds for motifs $H$ with a nontrivial decomposition, i.e., motifs that have more than a single component in their decomposition.

==> 800-lower_bounds.tex <==






Given a decomposition $\mathcal D$, we will create a subgraph $H_{\mathcal D}$ by adding edges to connect the components of $\mathcal D$ in a particular way.
Subsequently, our strategy will be to construct a family of graphs $G_{\mathcal D}(\vec z)$ on $n$ vertices and $m$ edges,
where $\vec z$ represents the set of intersections of an instance of the corresponding $\tSD$ problem.
Based on this family of graphs, we will show a lower bound on the query complexity of any algorithm that estimates $\cn H_{\mathcal D}$.
%Specifically, for graphs that contain $n$ vertices, $m$ edges, and $\cn O_k$ copies of the smallest odd cycle $O_i$,
%we obtain the following lower bound in \cref{thm:general_cycle_lower_bound}.
%\[
%\Omega\left( \sqrt m^k\cdot \frac{\cn O_k^r\cdot \prod_{i} \cn O_{k_i}\cdot \prod_{i} \cn S_{p_i}}{\cn H_{\mathcal D}}\right),
%\]


\subsection{Lower Bound Gadgets}
\label{sec:lower_bound_gadgets}

We use the following three types of gadgets for odd cycles $O_k$, and the last kind for stars $S_p$.
\begin{itemize}
    \item
\MM:
Given $\cn O_{k}$, this gadget is just a complete $k$-partite graph,
comprising of sets of vertices $ \langle R_1, R_2,\cdots, R_{k} \rangle$, each of size $\Theta(\cn O_{k}^{1/k})=  O(\sqrt m)$,
where each adjacent pair $R_i, R_{i+1}$ (as well as the pair $R_{k}, R_{1}$), induces a complete bipartite graph (\cref{fig:MM_gadget}).
Note that when $|R_i| = \sqrt m$, this gadget contains the maximum possible $\Theta(\sqrt{m}^{k})$ odd cycles.

    \item
    
    
\PP gadget:
Another type of gadget is similar to the \MM  has the same basic structure,
but with $|R_1| = 1$ (singleton vertex), and  $|R_j| = \Theta\left(\cn O_k^{1/(t-1)}\right)$ for all $j > 1$ (\cref{fig:PP_gadget}).
The connections between the sets also remain the same, which ensures that the total number of $t$-cycles created is $\Theta(\cn O_k)$.
This gadget cannot induce the maximum number of $t$-cycles,
which imposes the constraint $\cn O_k < \sqrt m^{t-1}$ (since we must have $|R_j|\cdot|R_{j+1}| < m$).
However, the advantage is that all the cycles created by this gadget share the singleton vertex in $R_1$.
This prevents the gagdet from \emph{inadvertently} creating copies of more complex subgraphs that contain multiple cycles of various sizes.
\todo{Move to next section}
    \item
\CC gadget:
This gadget is used to distinguish the two families of graphs, and therefore appears in two forms,
corresponding to the \YES and \NO instance of the $\tSD$ problem.
\tnote{TALYA: another attempt: 
The basic structure of this gadget contains the $k$-partite sets as before, but it also contains two additional sets $R_1', R_2'$. 
Between each $R_i$ and $R_{i+1}$ for $i>2$ there is a complete bipartite set, as well as between $R_k$ and $R_{i+1}$.
Now, there is no longer a complete bipartite set between $R_1$ and $R_2$, rather the edges between these sets as well as between the sets $R'_1$ and $R'_2$ are determined according to the instance $(\vec x, vec y)$ as follows.
For every $r_1^i, r_1^j\in R_1$, $r_2^i,r_2^j \in R_2$ there we add the  edges  $(r_1^i,r_2^j)$ and $(r_1^j,r_2^i)$ if and only if $\vec x_{ij}=\vec y_{ij}=1$.  Otherwise, we add the edges  $(r_1^i,(r'_2)^j)$ and $(r_1^j,(r_2')^i)$ to the gadget.
Hence, if $(\vec x, \vec y)$ is a \YES instance we get that the \CC gadget has $t\cdot \cn O_k^{(k-2)/k}$ odd cycles, and if it is a \NO instance then the gadget induces no cycles. 
}
Here, we present the latter, which contains the $k$-partite sets as before, but they also contain two additional sets $R_1', R_2'$,
which will be used to embed the $\tSD$ instance in \cref{sec:modifying_gadget_for_a_general_ksd_instance} (yielding the \YES version of the gadget).
Instead of a complete bipartite connection between $R_1\leftrightarrow R_2$,
there are (complete) connections between $R_1\leftrightarrow R_1'$ and $R_2\leftrightarrow R_2'$.
In this gadget, all the sets are of maximum size $\Theta(\sqrt m)$ (\cref{fig:CC_gadget_empty}).

    \item
\texttt{\SSS:}
Let $R_1$ be a set of of size $d_{avg} = m/n$, and let $R_2$ be a set of of size $\Theta\left( (\cn S_p / d_{avg})^{1/p}\right)$.
The gadget contains the complete bipartite set of edges $R_1 \leftrightarrow  R_2$.
(Observe that it always hold that $\cn s_p\leq m\cdot n^{p-1}$ and therefore $|R_2|\leq n$.)
\end{itemize}

%Before we present our main lower bound in \cref{sec:lower_bounds_for_the_case_where_the_decomposition_contains_a_cycle},
%we warm up by constructing a lower bound for the case when $\mathcal D$ is a collection of stars.

